Designing Topological Defect Lines Protected by Gauge-dependent Symmetry Indicators

Symmetry indicators are a modern tool for characterizing topological phases that require only minimal computational expense but provide an elegant means of designing practical devices. This paper demonstrates how a rotational symmetry indicator can be used to construct and characterize a topologically robust waveguide, which is then verified experimentally on a printed circuit board (PCB) platform. The design takes advantage of the real-space gauge-dependency of the symmetry indicators and adopts a $C_6$ lattice with simple shifts, forming a defect line supporting topological edge modes. It is shown that the modes can realize the same features as previous topological waveguides, but in addition possesses a greater degree of reconfigurability and the unique ability to form a one-way termination. Moreover, the design illustrates the critical role real space information plays in determining the topological properties of photonic crystals, enabling a wider range of possible realizations.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


